Markov invariants for phylogenetic rate matrices derived from embedded submodels

We consider novel phylogenetic models with rate matrices that arise via the embedding of a progenitor model on a small number of character states, into a target model on a larger number of character states. Adapting representation-theoretic results from recent investigations of Markov invariants for the general rate matrix model, we give a prescription for identifying and counting Markov invariants for such `symmetric embedded' models, and we provide enumerations of these for low-dimensional cases. The simplest example is a target model on 3 states, constructed from a general 2 state model; the `2->3' embedding. We show that for 2 taxa, there exist two invariants of quadratic degree, that can be used to directly infer pairwise distances from observed sequences under this model. A simple simulation study verifies their theoretical expected values, and suggests that, given the appropriateness of the model class, they have greater statistical power than the standard (log) Det invariant (which is of cubic degree for this case).

==> sec3.tex <==
\section{Linear invariants for the $\alpha=\beta$ case.}
In this section we show that for the $\alpha=\beta$ the model becomes diagonal and hence there are \emph{linear} Markov invariants.
The basic idea is to use the Hadamard inversion induced on symmetric tensors to give us a diagonalization of our $3\times 3$ rate matrix.
This model has as stationary distribution $\pi=(.25,.5,.25)$.
This is not too hard and we find the linear invariants:
\beqn
d_{22}&=4\left(f_{11}-f_{13}-f_{31}+f_{33}\right),\nonumber\\
d_{33}&=f_{11}-f_{12}+f{13}-f_{21}+f_{22}-f_{23}+f_{31}-f_{32}+f_{33},
\eqn 
with the theoretical values
\beqn
d_{22}&=2e^{-2(t_1+t_2)},\nonumber\\
d_{33}&=e^{-4(t_1+t_2)}.
\eqn

